Deep Academic Survey: Stateful Agentic Closed-Loop Paradigm for Academic Survey Automation

Academic surveys play a central role in organizing rapidly expanding scholarly literature, yet their construction requires extensive paper analysis, coherent knowledge organization, fine-grained citation support, and reliable manuscript assembly. Existing Deep Research and automated survey generation systems address parts of this process, but typically do not coordinate paper understanding, literature organization, evidence-grounded drafting, and manuscript validation through a shared, revisable state. We introduce DAS, a stateful agentic framework for generating publication-oriented academic surveys. Its key idea is to separate reusable paper analysis from topic-specific manuscript construction. DAS builds on DAS-2M, a dynamically updated metadata lake containing survey-oriented representations of approximately two million papers. Its agents maintain explicit literature, organization, writing, and finalization states through candidate-grounded taxonomy planning, reverse paper-to-section routing, and hierarchical claim and citation planning. Semantic review reactivates only the affected writing states for repair and reevaluation, forming a scoped closed loop with deterministic validation. We further introduce DAS-Bench, a 30-topic benchmark, together with DAS-Eval, which assesses scholarly citation quality, taxonomic synthesis, hierarchical discourse, and manuscript assembly reliability through 16 criteria. Among systems evaluated on all 30 topics, DAS achieves the highest average in all four dimensions, with an overall score of 4.34 compared with 4.03 for the strongest competitor, and the same ordering is preserved on the matched 21-topic CS subset. Blinded expert evaluation further prefers DAS to Naive RAG on 27 of 30 topics and to AutoSurvey on 19 of 21 shared CS topics. The project page is available at https://zhikaixu24.github.io/projects/DAS/.

==> table/main_results_cs21.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.05}
\setlength{\tabcolsep}{12pt}
\begin{tabular}{lc}
\toprule
Method & Total Avg.$\uparrow$ \\
\midrule
Human & 4.38 \\
\midrule
\textbf{\method{}} & \textbf{4.32} \\
Naive RAG & 3.96 \\
Gemini DR & 3.93 \\
InteractiveSurvey & 3.86 \\
SurveyForge & 3.78 \\
AutoSurvey & 3.73 \\
GPT DR & 3.71 \\
LiRA & 3.60 \\
Codex & 3.18 \\
\bottomrule
\end{tabular}
\caption{Matched comparison on the 21 CS topics shared by all evaluated systems. Human is reported for reference and excluded from system ranking.}
\label{tab:matched_cs_results}
\end{table}


==> table/profile_stage_ablation.tex <==
\begin{table}[!htbp]
\centering
\small
\renewcommand{\arraystretch}{1.08}
\setlength{\tabcolsep}{5.0pt}
\begin{tabular}{lcccc}
\toprule
Variant & BSC$\uparrow$ & TSQ$\uparrow$ & HDQ$\uparrow$ & MAR$\uparrow$ \\
\midrule
\textbf{Full \method{}}     & 3.85 & 4.22 & 4.28 & 5.00 \\
T/A at Retrieval      & 3.86 & 4.35 & 4.58 & 5.00 \\
T/A at Organization   & 3.85 & 4.22 & 4.33 & 5.00 \\
T/A at Drafting       & 3.75 & 4.36 & 4.44 & 5.00 \\
T/A Throughout        & 3.85 & 4.13 & 4.26 & 5.00 \\
\bottomrule
\end{tabular}
\caption{Stage-specific Paper Profile ablation on Bench-30. T/A denotes title and abstract input.}
\label{tab:profile_stage_ablation}
\end{table}

